On the robustness of the metric dimension of grid graphs to adding a single edge

The metric dimension (MD) of a graph is a combinatorial notion capturing the minimum number of landmark nodes needed to distinguish every pair of nodes in the graph based on graph distance. We study how much the MD can increase if we add a single edge to the graph. The extra edge can either be selected adversarially, in which case we are interested in the largest possible value that the MD can take, or uniformly at random, in which case we are interested in the distribution of the MD. The adversarial setting has already been studied by [Eroh et. al., 2015] for general graphs, who found an example where the MD doubles on adding a single edge. By constructing a different example, we show that this increase can be as large as exponential. However, we believe that such a large increase can occur only in specially constructed graphs, and that in most interesting graph families, the MD at most doubles on adding a single edge. We prove this for $d$-dimensional grid graphs, by showing that $2d$ appropriately chosen corners and the endpoints of the extra edge can distinguish every pair of nodes, no matter where the edge is added. For the special case of $d=2$, we show that it suffices to choose the four corners as landmarks. Finally, when the extra edge is sampled uniformly at random, we conjecture that the MD of 2-dimensional grids converges in probability to $3+\mathrm{Ber}(8/27)$, and we give an almost complete proof.

==> general/lowerbound.tex <==
% \newpage
\subsection{Lower bound on the decrease of the metric dimension}
\label{sec:lowerbound}

\begin{lemma}
Let $G = (V, E)$ be a connected graph, and let $G'$ be the graph obtained by adding edge $e$ between vertices $E$ and $F$ as before. Let $S$ be the resolving set of $G'$. Then, $S\cup \{E, F\}$ is the resolving set for $G$, and consequently $\beta(G) \le \beta(G')+2$.
\end{lemma}

\begin{proof}

Consider any pair of vertices $X$ and $Y$. Let $Z \in S$ be a vertex that distinguishes this pair in $G'$. There are three possibilities for where $X$ and $Y$ can be located: they can be both $N_Z$, both in $R_Z$, or (without loss of generality) $X \in R_Z$ and $Y \in N_Z$. Observe that if $Z$ is a normal vertex, then both $X$ and $Y$ must belong to $N_Z$, hence only Case 1 below is possible. If, however, $Z$ is not a normal vertex, then without loss of generality we can assume $Z \in R_E$. Now we treat the three cases for the location of $X$ and $Y$.

\textbf{Case 1:} $X$ and $Y$ both belong to $N_Z$.

    In this case, $d_{G'}(X, Z) = d_{G}(X, Z)$ and $d_{G'}(Y, Z) = d_{G}(Y, Z)$ so $Z$ will distinguish the pair in $G$ too.
   
 \textbf{Case 2:} $X$ and $Y$ both belong to $R_Z$.
 
Since we assumed $Z \in R_E$, by the anti-transitivity of special regions (Remark \ref{relation_classification}) $X, Y \in R_F$. Then, by Claim \ref{precise_distance},
\begin{align*}
d_{G'}(X, Z) &= XE + 1 + FZ,
\end{align*}
and similarly,
\begin{align*}
d_{G'}(Y, Z) &= YE + 1 + FZ.
\end{align*}
Since $d_{G'}(X, Z) \neq d_{G'}(Y, Z)$, we must also have $XE \neq YE$. Hence, $E$ will distinguish $X$ and $Y$ in $G$. 
    
\textbf{Case 3:} $X$ is in $R_Z$ and $Y$ is in $N_Z$.

Since we assumed $Z \in R_E$, we have that $X\in R_F$ by the anti-transitivity of special regions. By the definition of special and normal regions, we have
    \begin{align}
        \label{third_case_contra_1}
        XZ > d_{G'}(X,Z) \stackrel{\eqref{eq:precise_distance}}{=} XE + 1 +FZ \\ 
        \label{third_case_contra_2} YZ = d_{G'}(Y,Z) \stackrel{\eqref{eq:minAB}}{\leq} YE + 1 + FZ.
    \end{align}

 Assume that none of $Z$ and $E$ distinguishes $X$ and $Y$ in $G$. Then, $XE =YE$ and $XZ = YZ$, which clearly gives a contradiction between inequalities \eqref{third_case_contra_1} and \eqref{third_case_contra_2}. Hence, one of $Z$ and $E$ must distinguish $X$ and $Y$.  

\end{proof}


==> grid/atleast_4.tex <==
\begin{lemma}
\label{lem:MD4}
In addition to our main assumptions, if following conditions are satisfied then $\beta(G') = 4$:
\begin{equation}
    \label{assum1}
    Gain'\text{ is even}
\end{equation}
\begin{equation}
    \label{assum2}
    x_2 - x_1 \geq \frac{Gain'}{2} + 2
\end{equation}
\end{lemma}

\begin{figure}[!ht]
    \centering
    \includegraphics[scale = 0.75]{grid/big_grid.png}
    \caption{Grid partitioned into three regions $R_F$(pink), $N$(white) and $R_E$(blue) with important points marked}
\end{figure}

\begin{proof}
% Let $R_1 = R_R \cup R_S$, $R_2 = R_P \cup R_Q$. 
% We will refer $R_1$ and $R_2$ as special regions. It can b 
Assume that there exist three points $X$, $Y$, $Z$ that resolve the entire graph. 

% \begin{claim}
% $Gain(A, B)$ is even for any pair of vertices $A$ and $B$.
% \end{claim}
% \begin{proof}

% \end{proof}

% \begin{claim} \label{boundary}
% % There must be at least $2$ points on the boundary of the grid such that they are on opposite boundaries and they are not opposite corners. 
% Out of these 3 points, some 2, say $X$ and $Y$, must satisfy following:
% \begin{enumerate}
%     \item They are on opposite boundaries 
    
%     \item If one of them is a corner, other must be the adjacent corner
% \end{enumerate}
% \end{claim}
% \begin{proof}
% Consider vertices $A(1, 2)$ and $B(2, 1)$. It is easy to see that only vertices on boundaries $PQ$ and $PS$ except corner $P$ will be able to distinguish $X$ and $Y$ as none of $E$ and $F$ is on boundary. So we need at least one point from union of boundaries $PQ$ and $PS$ except $P$. Similarly for other $4$ corners. (explain more)
% \end{proof}

% $Gain(A, B)$ between any pair of vertices $A$ and $B$ is defines as $AB - d_{G'}(A, B)$. Informally it is the reduction in the distance on adding the edge $e$.

\begin{claim} \label{atmostone}
% At most one point can lie in a special region.
$R_E$ and $R_F$ can contain at most one point from $X$, $Y$, $Z$
\end{claim}
\begin{proof}
Assume that two points lie in $R_E$. Since Gain for any point in $R_E$ is even, it is at least 2. Consequently, neighbours of $E$ i.e $E_1, E_2, E_3, E_4$ will have same distance from those two points and by Remark \ref{four_points}, a single point cannot distinguish these $4$ points. 
% Now using only one point we have to distinguish these $4$ points. Clearly this third point cannot be in $R_1$. So for remaining possibilities of the third point, distances from all $E_i$ will be same as that in the normal grid. As a result, it cannot be in rectangle formed by points $E$, $(n, y_1)$, $R$, $(x_2, m)$ as otherwise $E_1$ and $E_2$ will not be distinguished. Similarly it cannot be in rectangles formed by $E$, $(x_2, m)$, $S$, $(1, y)$ and $E$, $(1, y_2)$, $P$, $(x_2, 1)$ and $E$, $(x_2, 1)$, $Q$, $(n, y_2)$. Basically it cannot be anywhere in the grid. Hence we can't have two points in the same special region.
\end{proof}
Based on the claims \ref{boundary} and \ref{atmostone}, there are various possibilities for the three points:

\begin{figure}[!ht]
    \centering
    \includegraphics[scale = 0.15]{case-tree.jpg}
    \caption{"case tree" for proving Lemma 6}
    \label{fig:big_tree}
\end{figure}

\begin{enumerate}


% case 2:
\item
First point $X(1, k_1)$ lies on boundary $PS$ in $R_2$ and second point $Y(n, k_2)$ lies on boundary $QR$ in $R_1$.
% i.e. above $(n, \beta)$. 
By claim $\ref{atmostone}$, third point $Z$ must belong to the normal region. 
\begin{enumerate}
% sub-case 1: 
\item
$k_1 < k_2$ \\
See that the pairs $((n-1, k_2), (n, k_2 -1))$ and $((1, k_1 +1 ), (2, k_1))$ are not distinguished by $X$ and $Y$(as $E$ and $F$ are not on boundaries). And only one point in normal region cannot distinguish both pairs hence this sub-case is not possible.
% sub-case 2:
\item
$k_1 = k_2 = k$ \\
Clearly $\alpha + 1 \leq k \leq \beta - 2$. Let $Z = (i, j)$. As $Z \in N$, $\alpha - 1 \leq j \leq \beta$. Let's consider the case when $j < k$. Let $\gamma = \frac{(y_1 - y_2) - (x_2 - x_1) + 1}{2}$. Note that $\gamma = \frac{Gain' + 2}{2} \geq 2$. We claim that two points $T(n, j - \gamma)$ and $W(n + j - k, \gamma + k)$ are not distinguished by $X, Y, Z$. Using ranges of $k$ and $j$ as mentioned above and substituting the values of $\alpha$, $\beta$, $\gamma$ it can be verified easily that $T$ and $W$ are valid points on the grid.\\
\begin{itemize}
    \item 

First we check with point $Z$. \\
As it is a normal point, $$d_{G'}(T, Z) = (n - i + \gamma)$$ Now, as $j < k$, maximum value of $i - j$ is attained at point $(x_1, \alpha - 1)$ i.e. $$i-j \leq x_1 - \alpha + 1$$ And $$n - (\beta - 1) \leq n - k$$ But 
\begin{align}
    n - \beta + 1 - (x_1 - \alpha + 1) &= n - x_2 \\
        &\geq 0
\end{align}
Hence $i - j \leq n - k$ which implies\\ $d_{G'}(Z, W) = |n - k - (i - j)| + |\gamma + k - j| = (n - i + \gamma) = d_{G'}(T, Z)$ 

\item
Next we check with point $X$. \\
% As $j \geq \alpha + 1$, it can be proved that $j - \gamma \geq y_2$, also it can be proved that $j - \gamma < (y_2 + \frac{Gain_{max}(X)}{2})$ hence \begin{align}
%     d_{G'}(X, T) &= TX - Gain(T, X) \\
%     & = (n - 1 + \gamma + k - j) - 2*(\frac{Gain_{max}(X)}{2} + y_2 - (j - \gamma))\\
%     & = n - 1 + \gamma + j - k
% \end{align}
%  And it can be proved that $$y_2 + \frac{Gain_{max}(X)}{2} \leq \gamma + k$$ hence $W$ lies outside of special region of $X$ so $d_{G'}(W, X) = WX = n + j - k - 1 + \gamma$. Hence, $d_{G'}(W, X) = d_{G'}(Z, X)$.
By claim \ref{special_region} we know that highest y-coordinate of a point in special region of $X$ will be 
\begin{align}
    y_h = &y_2 + \frac{Gain_{max}(X)}{2} - 1\\ & = y_2 + \frac{Gain}{2} - (y_1 - k) - 1\\& = k - 2 - \frac{Gain'}{2} \\& = k + \gamma - Gain' - 3\\ & > k + \gamma\\
\end{align}
Hence $W$ will be out of the special region of $X$ which gives $$d_{G'}(X, W) = WX = |n + j - k - 1| + |\gamma + k - k| = n + j - k - 1 + \gamma$$
Now, as 
\begin{align}
    j & \leq k - 1,\\
    j - \gamma & \leq k - \gamma - 1\\
    & = k - 2 - \frac{Gain'}{2}\\
    & = y_h
\end{align}
Hence $T$ lies inside special region of $X$. This implies
\begin{align}
    d_{G'}(X, T) &= TE + 1 + FX\\
    & = (n - x_2) + |j - \gamma - y_2| + 1 + (x_1 - 1) + (y_1 - k)\\
\end{align}
Using $j \geq \alpha$ it is easy to show that $j - \gamma \geq y_2$. This gives $$d_{G'}(X, T) = (n - x_2) + (j - \gamma - y_2) + 1 + (x_1 - 1) + (y_1 - k) = n + j - k - 1 + \gamma = d_{G'}(X, W)$$

\item
Finally we check with point $Y$. \\
$d_{G'}(Z, T) = k - j + \gamma$ is clear. Now we will show that $W$ will be outside the special region of $Y$. For this, we will show that the $\gamma + k$ is less than the lowest y-coordinate of the special region of $Y$. By claim \ref{special_region} the lowest y-coordinate of $R_Y$ is 
\begin{align}
    y_l = & y_1 - \frac{Gain_{max}(Y)}{2} + 1\\
    & = y_1 - (\frac{Gain}{2} - (k - y_2)) + 1\\
    & = k + \gamma + 1
    & > k + \gamma
\end{align}
Hence, $$d_{G'}(Z, W) = (n - (n + j - k)) + (\gamma) = k - j + \gamma = d_{G'}(Z, T)$$
\end{itemize}
Now due to $180^o$ symmetry, for $j > k$ also we can find two points similarly.  

When $j = k$, points $(n, k-1)$ and $(n, k+1)$ cannot be distinguished and can be proved easily. \\ \\
Hence this case is also not possible. 

% sub-case 3:
\item
$k_1 > k_2$.
\begin{enumerate}
    \item
% sub-sub-case 1:
$k_1 > y_1$ or $k_2 < y_2$ i.e. $X$ is below $H$ or $Y$ is above $M$. \\  Let's say $Y$ is above $M$. Pair $((n-1, k_2), (n, k_2+1))$ will not be distinguished and it also cannot be distinguished by any normal point except the two on the boundary $QR$. But this case is already covered when point on boundary $PS$ is in region $R_2$ and point on the opposite boundary is a normal point. 
\item
% sub-sub-case 2:
$k_1 \leq y_1$ and $k_2 \geq y_2$ and $k_1 - k_2 > 1$. \\ 
% We analyse the special regions of $X$ and $Y$. $Gain$ for $X$ is $G_1 = EX - (1 + FX) = 2k_1 + x_2 - x_1 - y_1 - y_2 - 1$. The lowest $x$-coordinate of a point in the special region of $X$ will be therefore $x_{t1} = x_2 - \frac{G_1}{2} +1 = \frac{y_1 + y_2 + x_1 + x_2  - 2k_1 + 3}{2}$.
By claim \ref{special_region} we can infer that lowest x-coordinate of the special region of point $X$ is 
\begin{align}
    x_{lx} & = x_2 - \frac{Gain_{max}(X)}{2} + 1\\
     & = x_2 - (\frac{Gain}{2} - (y_1 - k_1)) + 1\\
\end{align}
It can be seen that pair $((x_{lx}, y_2 - 1), (x_{lx} - 1, y_2))$ is not distinguished by $X$ and $Y$(\textbf{why, explain more}) and no normal point with $x$-coordinate greater than or equal to $x_{lx}$ can distinguish this pair. Symmetrically, highest x-coordinate of special region of $Y$ will be 
\begin{align}
    x_{ly} & = x_1 + \frac{Gain_{max}(Y)}{2} - 1\\
     & = x_1 + (\frac{Gain}{2} - (y_2 - k_2)) - 1\\
\end{align}
Again, pair $((x_{ly}, y_1 + 1), (x_{ly} +1, y_1))$ 
% with $x_{t2} =\frac{y_1 + y_2 + x_1 + x_2 - 2k_2 - 1}{2}$
is not yet distinguished and no normal point with $x$-coordinate less than or equal to $x_{t2}$ is able to distinguish this pair. But for $k_1 - k_2 \geq 2$, $x_{t1} \leq x_{t2}$ hence all normal points are eliminated and so this case is not possible.
\item
% sub-sub-case 3:
$k_11 \leq y_1$ and $k_2 \geq y_2$ and $k_1 - k_2 = 1$. \\ 
Let $k_1 = k$. $Gain$ for $X$ is $G_X = 2k + x_2 - x_1 - y_1 - y_2 - 1$. Hence lowest y-coordinate of the special region of $X$ is $y_t = y_2 + \frac{G_X}{2} - 1 = (k - 1) + \frac{(x_2 - x_1) - (y_1 - y_2) - 1}{} < (k - 1)$. Hence the points $(n, k)$ and $(n-1, k-1)$ lie in the normal region for point $X$ and hence not yet distinguished. Also no normal point in the rectangle $R_3$ formed by points $(n-1, k), (n-1, m), (1, m), (1, k)$ can distinguish this pair. Similarly it can be proved that points $(2, k)$ and $(1, k-1)$ are in the normal region of point $Y$ hence they are not yet distinguished and also cannot be distinguished by any normal point in the rectangle $R_4$ formed by points $(2, k-1), (n, k-1), (n, 1), (1, 1)$. So only normal points on boundary are left to be considered but that is already seen in the case when one point is in $R_2$ and other point is on opposite boundary in the special region. Hence we are done with this case. 
\end{enumerate}
\end{enumerate}

%case-2
\item
First point $X(1, k)$ which is on the boundary $PS$ belongs to $R_1$. \\ Then, one of the remaining two points must lie on boundary $QR$ below $(n, \beta - 1)$ by claims \ref{atmostone} and \ref{boundary}.
% sub-case 1 : 
\begin{enumerate}
\item 
% sub-case 1
second point is not $(n, \beta)$. Then, pairs $((2, \alpha), (1, \alpha + 1))$ and $((n, \beta), (n-1, \beta +1))$ are not distinguished by these points and a single point cannot distinguish both of them.
% sub-case 2 :
\item
second point is $(n, \beta)$. Now $(1, k+1)$ and $(2, k)$ are not distinguish and none of the points in normal region can distinguish them except $(1, \alpha)$ and $(1, \alpha +1)$. But if we choose these points, $(x_2 - 1, \beta)$ and $(x_2, \beta - 1)$ are still not distinguished.
Hence, this case is not possible. 
\end{enumerate}


% case 3:
\item
$X(1, k_1)$ is in $R_2$ and $Y(n, k_2)$ is in normal region. Clearly $k_2 < y_1$.
\begin{enumerate}
\item
% sub-case 1:
$k_1 < k_2$. As $k_2 < y_1$, $k_1 < y_1$ so the special region of $X$ will be strictly less than the $\beta$. Hence the pair $((n, k_2 - 1), (n-1, k_2))$ cannot be distinguished by $X$ and $Y$ and also cannot be distinguished by any point in the rectangle region formed by points $(n-1, k_2 - 1), (1, k_2 - 1), (1, 1), (n-1, 1)$. So only points remaining are those above $k_2 - 1$ on boundary $QR$. But, pair $((x_2, 1), (x_2 - 1, 2))$ also is not distinguished by $X$ and $Y$ and it cannot be distinguished by any point on boundary $QR$ except the corner $Q$. So only case remaining is when third point is corner $Q$. But if we take these three points, pair $((1, k_1+1), (2, k_1))$ cannot be distinguished by any of them. Hence this case is not possible. 
\item
% sub-case 2[add figure]:
$k_1 = k_2 = k$. $k$ can take two values: $\beta$ and $\beta + 1$. Hence $k \geq \beta$. Hence $Gain$ of $X$, $G_1 = EX - (1 + FX) = 2k_1 + x_2 - x_1 - y_1 - y_2 - 1 \geq 2\beta + x_2 - x_1 - y_1 - y_2 - 1 = 2(x_2 - x_1 - 1)$. Hence the highest y-coordinate of the special region of $X$ will be $y_t = y_2 + \frac{G_1}{2} - 1 \geq y_2 + x_2 - x_1 - 2$. Now pair $((n, y_t), (n-1, y_t+1))$ cannot be distinguished by $X$ and $Y$ and also by any point in the region formed by rectangle $(n-1, y_t), (1, y_t), (1, 1), (n-1, 1)$. Let's call this rectangle as $R_3$. \\ \\
Similarly lowest x-coordinate of the special region of $X$ will be $x_t = x_2 - \frac{G_1}{2} + 1 \leq x_1 + 2$ and pair $((x_t - 1, 2), (x_t, 1))$ also cannot be distinguished by $X$ and $Y$ and the rectangle, let's name it $R_4$. Now we try to show that $R_1 \setminus \{Q\} \subseteq R_3 \cup R_4$. \\
\begin{align}
\alpha - 1 & = \frac{y_1 + y_2 + x_1 - x_2 - 1}{2} - 1 \\
 & = (\frac{y_1 - y_2 + x_1 - x_2 - 1}{2} + 1 - (x_2 - x_1)) + (y_2 + x_2 - x_1 - 2) \\
 & < y_2 + x_2 - x_1 - 2 \text{ (By our assumption)}\\
 & \leq y_t
\end{align}
So,  $\alpha - 1 < y_t$ which implies that $R_R \subset R_3$. \\
Now we will find the intersection of the boundary of $R_S$ and $R_3$ which is not on the boundary of main grid of course. As, $\alpha - a < y_t \leq \beta$, this intersection must be on the diagonal part of $R_S$. For all points in this diagonal $D(a, b)$, \begin{align}
  a - b & = x_2 - \frac{Gain_{max}}{2} + 1 - y_2 \\
  & = \frac{x_1 + x_2 - y_1 - y_2 + 3}{2}
\end{align}Hence the x-coordinate of the required intersection point will be \begin{align}
    \delta & = y_t + \frac{x_1 + x_2 - y_1 - y_2 + 3}{2} \\ 
    \geq \frac{3x_2 - x_1 + y_2 - y_1 - 1}{2}
\end{align}.
If $\delta \geq x_1 + 1$ is true than entire $R_1$(except corner $Q$) will be inside the union of rectangles $R_3$ and $R_4$ as $x_t \leq x_1 + 2$. Indeed, 
\begin{align}
    \delta - x_1 - 1 & \geq \frac{3x_2 - 3x_1 + y_2 - y_1 - 3}{2} \\
    & \geq x_2 - x_1 - (\frac{y_1 - y_2 + x_2 - x_1 - 1}{2} - 2 \\
    & \geq 0\text{  (By our assumption)}
\end{align}
Hence we proved that third point cannot be taken inside region $R_1$ except the corner $Q$. But if we take $Q$ then points $A=(x_1+k-\alpha-1, k+1)$ and $B=(x_1 + k - \alpha -1, k-1)$ cannot be distinguished. This is because $A$ and $B$ are normal points for both $X$ and $Q$ so distance from them to $A$ and $B$ are same. Point $A$ lies on the boundary of special region of $Q$ as $A_x - A_y = x_1 - (\alpha + 2)$ hence $Gain(A, Q) = 2$. Now since $BQ- AQ = 2$, clearly $d_{G'}(A, Q) = d_{G'}(B, Q)$. Hence third point cannot be in $R_1$ so it has to be in normal region. But if we take $(i, j)$ as third point in normal region then points $Z(n, j - \gamma)$ and $W(n + j - k, \gamma + k)$ cannot be distinguished. This can be verified very similarly as above and it is also easier as two points are normal points.
\item
% sub-case 3: 
$k_1 > k_2$. \\
Here $k_1 \geq \beta + 1$ so now $y_t \geq y_2 + x_2 - x_1 - 1$ and $x_t \leq x_1 + 1$. Again, of course $R_1\setminus\{Q\}$ will be subset of $R_3 \cup R_4$, but in this case, normal region will also be a subset of $R_1\setminus\{Q\}$. This is because \begin{align}
    y_t & \geq y_2 + x_2 - x_1 - 1 \\
    & \geq \frac{1 + y_2 + y_1 +x_1 - x_2}{2}\text{  ...(By our assumption)} \\
    & = \alpha + 1
\end{align}Hence the rectangle formed by $(1, \alpha), (1, \alpha + 1), (x_1, \alpha), (x_1, \alpha + 1)$ is a subset of $R_3$. Now, the remaining points in the normal region has x-coordinate $\geq x_1 + 1$ and as $x_t \leq x_1 + 1$, these normal points will lie in $R_4$. Hence it is established that normal region is a subset of $R_3 \cup R_4$ which means only remaining point is $Q$ but then the pair $((n, k_2+1),(n-1, k_2))$ will not be distinguished. Hence, this sub-case is not possible. 
\end{enumerate}

%case N-N:
\item 
$X(1, k_1)$ lie on boundary $PS$ in normal region $N$ and $Y(n, k_2)$ lies on boundary $QR$ in normal region $N$\\

$k_1$ is either $\alpha$ or $\alpha + 1$ and $k_2$ is either $\beta$ or $\beta + 1$. 
As $\alpha + 1 < \beta$, pair $((n-1, \beta), (n, \beta - 1))$ is not distinguished by $X$ and $Y$ and cannot be distinguished by any point which belongs to both, the rectangle formed by opposite corners $(n-1, \beta - 1)$, $(1, 1)$ and $R_1 \cup N$.\\

Similarly, pair $((1, \alpha + 2), (2, \alpha + 1))$ is not distinguished and cannot be distinguished by any point which belongs to (rectangle formed by opposite corners $(2, \alpha + 2)$ and $(n, n)$) $\cap$ ($R_2 \cup N$). This leaves out the points which are on boundary $QR$ in $R_1$ and on $PS$ in $R_2$. But if we take $Z$ from either of these possibilities, this case is already covered when $X$ is in $R_2$ and $Y$ is in $N$.  
% case 5:
\item
$X(k_1, 1)$ is on boundary in $PQ$ and $Y(k_2, n)$ is on boundary $RS$. Third point must be in normal region.
\begin{enumerate}
\item 
% sub-case 1:
$k_2 < x_1$ or $k_1 > x_2$ 
We consider only $k_2 < x_1$. Same arguments work for $k_1 > x_2$ due to $180^{\circ}$ symmetry. 
\begin{enumerate}
\item 
% sub-sub-case 1 :
$k_1 > k_2$. Pair $((k_2+1, n), (k_2, n-1))$ is not yet distinguished and cannot be distinguished by any normal point with x-coordinate greater than $k_2$. 
Also pair
% $((k-1, y_1), (k, y_1 -1))$ 
$((k_2, \alpha - 1), (k_2 + 1, \alpha))$
is not yet distinguished and cannot be distinguished by any normal point with x-coordinate less than $k_2+1$.
% So we are left with normal points having x-coordinate $k$. But if we choose third point as $(k, j)$ then pair $((k+1, j), (k, j-1))$ will not be distinguished by any three of them.
Hence this sub-sub-case is not possible. \item
% sub-sub-case 2: 
$k_1 < k_2$. Pair $((k_1+1, 1), (k_1, 2))$ is not distinguished yet and it cannot be distinguished by any normal point with x-coordinate more than $k_1$. Pair $((k_2, \alpha + 1), (k_2-1, \alpha + 2))$ is not yet distinguished and no normal point with x-coordinate less than $k_2$ can distinguish it and $k_1 < k_2$ so this sub-sub-case is also not possible. 
\item
% sub-sub-case 3: 
$k_1 = k_2 = k$. Pair $(F_2, F_3)$ is still not distinguished and no normal point with x-coordinate $\geq x_1$ so only normal points remaining to be considered are those which have x-coordinate less than $x_1$ and so they have y-coordinate either $\alpha$ or $\alpha + 1$. But if we choose any such point as our third point, we cannot distinguish the pair $(O, (n-1, \alpha))$ hence this sub-sub-case is also not possible. \\
\end{enumerate}
Hence, this sub-case is not possible. 
\item
% sub-case-2:
$k = x_1$ or $k_1 = x_2$. No normal point can distinguish all three pairs $(F_1, F_4)$, $(F_1, F_2)$ and $(F_2, F_4)$ hence this sub-case is not possible. 
% \item
% sub-case-3[check if can be combined]: 
% $k = 1$. Pair $((2, m), (1, m-1))$ cannot be distinguished by any normal point except the two on the border $PS$. But If we choose one of these two points and if $Y$ is not the corner $Q$, again pair $((n-1, \alpha), O)$ cannot be distinguished by any of the three. So only possibility remaining is $Y$ being corner $Q$. But then, pair $((n-1, 1), (n, 2))$ cannot be distinguished. Hence this sub-case is not possible.
\item
% sub-case-4:
$x_1 < k_2$ and $k_1 < x_2$. \\
% If $k' \geq x_2$, that case is already covered due to $180^{\circ}$ symmetry. 
By claims \ref{boundary} and \ref{atmostone} it can be infered that none of $X$ and $Y$ can be corners. 
We know that $R_P$ is a subset of the special region of the points on boundary $PQ$ having x-coordinate less than or equal to $x_2$. As a result, Pairs $((k_2+1, y_1), (k_2, y_1 - 1))$ and $((k_2-1, n), (k_2, n-1))$ cannot be distinguished by $X$ and $Y$. Also no normal point except the ones having x-coordinate $k$ can distinguish both of these pairs. Hence only possibility remaining is when $Z$ has x-coordinate $k_2$. Now there are three possibilities for $Y$:
\begin{enumerate}
\item 
% sub-sub-case 1: 
$k' > k$. \\ Then, pair $((k'- 1, y_2), (k', y_2+1))$ remain undistinguished.(remember that we are only considering $k' < x_2$)
\item
% sub-sub-case 2:
$k' < k$. \\ Then, pair $((k'+1, 1), (k', 2))$ cannot be distinguished as $R_R$ will be the subset of special region of $X$ as shown above.
\item
% sub-sub-case 3:
$k' = k$. \\ Let the third point, i.e the point in the normal region be $Z(k, j)$. As $x_1 < k = k' < x_2$, special region is "thinner" then the maximum value, hence points $(k+1, j)$ and $(k-1, j)$ will be outside the special region of both $X$ and $Y$ as they just touch the maximum special region. \\ \\

\end{enumerate}
\end{enumerate}
\end{enumerate}

Thus we have checked every possibility and three points are not sufficient to distinguish all pairs of vertices. 

\end{proof}

==> grid/counting.tex <==
\begin{proof}[Proof of Theorem \ref{thm_grid_random}]

There are $(n- a - 1)(n - b - 1)$ possible edges with $x_2 - x_1 = a$ and $y_1 - y_2 = b$ which satisfies all the assumptions, i.e. $a > 0$, $b > 0$, $b > a$ and none of the endpoint is on boundary of the grid.

First we calculate the number of possible edges such that $\beta(G') = 4$. By lemma \ref{}, additional conditions that needs to be satisfied are $b - a$ is odd, $b - a \geq 3$ and $a \geq \frac{b - a - 1}{2} + 2$ which reduces to $a \geq \frac{b}{3} + 1$. Now $1 \leq a, b \leq n - 2$ so total number of possible edges is 
     $$\sum_{i = 1}^{\floor{\frac{n - 5}{3}}} \sum_{b = 3(i + 1)}^{n - 2} (n - b + 2i)(n - b - 1)$$
     
    which reduces asymptotically to $$\frac{1}{27}n^4 + \theta(n^3)$$. Total number of possible edges for a $n \times n$ grid with conditions $a > 0$, $b > 0$, $b - a \geq 3$ and endpoints not lying on boundary is $\frac{n^4}{8} + \theta(n^3)$. Hence, \begin{align}
        P(\beta(G') = 4)  & = \frac{\frac{1}{27}n^4 + \theta(n^3)}{\frac{n^4}{8} + \theta(n^3)} \\
        & = \frac{8}{27}
    \end{align}Which completes the proof. 
    
\end{proof}

==> ring/ring.tex <==
\section{Ring graph}
\label{sec:ring_graph}

It is well-known that the metric dimension of a ring graph on $n$ nodes is two. A set of any two adjacent vertices is a resolving set. In this section we will see that metric dimension will remain two on adding an edge between any two vertices. Hence, this is an example of a graph whose metric dimension cannot be changed by adding an edge.


\begin{figure}[!ht]
    \centering
    \includegraphics[scale = 0.4]{ring/ring_one.png}
    \caption{Ring with an additional edge. Vertices $X$ and $Y$ marked as blue points form a resolving set.}
    \label{fig:my_label}
\end{figure}


\begin{theorem}
Let $G$ be a ring with $n$ vertices. $G'$ is obtained by adding an edge between any two vertices of $G$. Then, the metric dimension of $G'$ is exactly two. 
\end{theorem}

\begin{proof}
Let us denote the vertices of $G$ by $A_1, \dots, A_n$. Without loss of generality, let one endpoint of the extra edge be $A_1$ and the other be $A_x$ with $1 < x < n$. It is well-known (see e.g. \cite{chartrand2000resolvability}) that the metric dimension of any graph that is not a path is at least two. We show that set of vertices $X=A_{\floor{\frac{x}{2}}}$ and $Y=A_{\floor{\frac{x}{2}}+1}$ is a resolving set for $G'$ which proves that metric dimension is exactly two.

We distinguish two cases based on the parity of $x$.

\textbf{Case 1:} $x$ is even:

In this case, 
\begin{align*}
|d_G(A_1, X) - d_G(A_x, X)| &= \left|\min\left( \frac{x}{2} -1 , n-\frac{x}{2}+1\right) - \min\left( x-\frac{x}{2}, n-x+\frac{x}{2}\right)  \right| \\
&= \left| \left(\frac{x}{2}-1\right)-\left(x-\frac{x}{2}\right) \right| =1,
\end{align*}
and 
\begin{align*}
|d_G(A_1, Y) - d_G(A_x, Y)| &= \left|\min\left( \frac{x}{2} , n-\frac{x}{2}\right) - \min\left( x-\frac{x}{2}-1, n-x+\frac{x}{2}+1 \right)  \right| \\
&= \left| \left(\frac{x}{2} \right)-\left(x-\frac{x}{2}-1\right) \right| =1.
\end{align*}
By Claim \ref{partition}, both $X$ and $Y$ are normal vertices. Consequently, the extra edge has no effect on distances of any vertex from $X$ and $Y$. Since a set of two adjacent vertices is a resolving set for a ring, the set $\{X, Y\}$ is a resolving set for $G'$ too.  

\textbf{Case 2:} $x$ is odd:

In this case,
\begin{align*}
|d_G(A_1, X) - d_G(A_x, X)| &= \left|\min\left( \frac{x-1}{2} -1 , n-\frac{x-1}{2}+1\right) - \min\left( x-\frac{x-1}{2}, n-x+\frac{x-1}{2}\right)  \right| \\
&= \left| \left(\frac{x-1}{2}-1\right)-\left(x-\frac{x-1}{2}\right) \right| =2,
\end{align*}
and 
\begin{align*}
|d_G(A_1, Y) - d_G(A_x, Y)| &= \left|\min\left( \frac{x-1}{2} , n-\frac{x-1}{2}\right) - \min\left( x-\frac{x-1}{2}-1, n-x+\frac{x-1}{2}+1 \right)  \right| \\
&= \left| \left(\frac{x-1}{2} \right)-\left(x-\frac{x-1}{2}-1\right) \right| =0.
\end{align*}

By Claim \ref{partition}, $Y$ is a normal vertex and $X$ is not. By Remark \ref{gain_max_remark}, 
\begin{equation}
    \label{eq:ring_proof_Gm1}
\Gain_{\max}(X) = \max(0,|d_G(A_1, X) - d_G(A_x, X)| - 1) = 1,
\end{equation}
or equivalently $0 \leq \Gain(A, X) \leq 1$ for any vertex $A$ in the ring.

Suppose for contradiction that there exist two nodes $M$ and $N$ that are distinguished by neither $X$ nor $Y$ in $G'$, i.e., $d_{G'}(M, X) = d_{G'}(N, X)$ and $d_{G'}(M, Y) = d_{G'}(N, Y)$. Then, since $Y$ is a normal vertex, we must have $d_{G}(M, Y) = d_{G}(N, Y)$, and since we also know that $\{X, Y\}$ is a resolving set in $G$, we must have $d_{G}(M, X) \ne d_{G}(N, X)$. Let $d_G(M,X)<d_G(N,X)$ without loss of generality, and let us denote $k=d_G(M, Y) = d_G(N, Y)$. Next, we compute the distances between $X$ and $M,N$. Since $M$ and $N$ are equidistant from $Y$ in $G$, and $X$ is the neighbor of $Y$ that is closer to $M$, $X$ must on the shortest path between $Y$ and $M$ in $G$, and therefore we must have $d_G(M, X) = k - 1$. Now we have two cases: either $Y$ is  on the shortest path between $X$ and $N$, in which case we must have $d_G(N, X) = k + 1$, or $Y$ is not on the shortest path between $X$ and $N$, which is only possible if $X$ and $Y$ are the two farthest vertices from $N$, which further implies that $d_G(N, X)=d_G(N, Y)=k=(n-1)/2$, with $n$ odd. We treat these sub-cases separately.
% Given that $M$ and $N$ are equidistant from $Y$ in the original ring, absolute difference between $d_G(M, X)$ and $d_G(N, X)$ can be either $1$ or $2$. When $n$ is odd and $M$, $N$ are the two farthest vertices from $Y$, the absolute difference will be $1$ and it is easy to see that in all other cases, it will be $2$. Hence, depending on the value of $|d_G(M, X) - d_G(N, X)|$, we have two sub-cases here. 

\textbf{Sub-case 1:} $d_G(N, X)=k$

This sub-case is only possible for $n$ odd and $k = (n - 1)/2$, which means that that $M$ and $N$ are the two farthest vertices from $Y$, and are therefore adjacent. Also $A_1$ must be on the $YM$ half, and $A_x$ must be on the $YN$ half of the ring. Since the pairs of vertices $(M,N)$ and $(A_1, A_x)$ are both equidistant from $Y$, the distance between $M$ and $A_1$ and the distance between $N$ and $A_x$ will also be equal in $G$. Formally, we write 
\begin{equation*}
\label{eq:ring_proof_MANA}
    d_G(M, A_1) = d_G(M, Y) - d_G(A_1, Y) = d_G(N, Y) - d_G(A_x, Y) = d_G(N, A_x).
\end{equation*}
Since $A_1$ is on the $YM$ half, and $A_x$ is on the $YN$ half of the ring, the shortest path between $M$ and $A_x$ must go through $N$, and the shortest path between $N$ and $A_1$ must go through $M$. We also know that $M$ and $N$ are adjacent, and therefore
\begin{equation}
\label{eq:ring_proof_MA1}
|d_G(M, A_1) - d_G(M, A_x)| = |d_G(M, A_1) - (d_G(N, A_x)+1)| =1,
\end{equation}
and
\begin{equation}
\label{eq:ring_proof_MA2}
|d_G(N, A_1) - d_G(N, A_x)| = |(d_G(M, A_1)+1) - d_G(N, A_x)| =1.
\end{equation}
Equations \eqref{eq:ring_proof_MA1} and \eqref{eq:ring_proof_MA2}  show, by Claim \ref{partition}, that $M$ and $N$ are normal vertices. Hence, $$|d_{G'}(M, X) - d_{G'}(N, X)| = |d_G(M, X) - d_G(N, X)| = |(k-1)-k| = 1,$$ contradicting the assumption  $d_{G'}(M, X) = d_{G'}(N, X)$.

\textbf{Sub-case 2:} $d_G(N, X)=k+1$

% Consequently, since $X$ and $Y$ are adjacent vertices, \begin{equation}\label{contra}
%     |d_G(M, X) - d_G(N, X)| = 2.
% \end{equation}
Since $\Gain_{\max}(X)=1$ by equation \eqref{eq:ring_proof_Gm1}, we have:
\begin{equation}
\label{gain_lt_1}
   0 \leq d_G(M, X) - d_{G'}(M, X) \leq 1,
\end{equation}
and
\begin{equation}
\label{gain_lt_2}
   0 \leq d_G(N, X) - d_{G'}(N, X) \leq 1.
\end{equation}
Inequalities \eqref{gain_lt_1} and \eqref{gain_lt_2}, with the assumption of $d_{G'}(M, X) = d_{G'}(N, X)$, imply that $$-1 \leq d_G(M, X) - d_{G}(N, X) \leq 1,$$ which is impossible because previously we had $d_G(N, X)=k+1$ and $d_G(M, X) = k-1$.

Hence, all pairs of nodes are distinguished by $X$ and $Y$, and the proof is completed.
\end{proof}


==> ring/ring_extra_edge1.tex <==
% This is an example of a graph for which metric dimension cannot be increased by adding a single edge.



% \end{document}

==> ring/ring_multiple.tex <==
Here we give an upper bound on the metric dimension of the graph obtained by adding multiple edges to a ring. 

\begin{figure}[!ht]
    \centering
    \includegraphics[scale = 0.5]{ring_multi.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

\begin{theorem}
Let $G$ be a ring graph. We add $k$ distinct edges randomly in $G$ to obtain graph $G'$. Then, metric dimension of $G'$ is at most $4k$.  
\end{theorem}

\begin{proof}
% For every extra edge, add both neighbours of both the endpoints in the resolving set.
Let $R$ be the set of neighbours of the endpoints(on the ring, not the other endpoint) of the extra edges. Formally, 

$$R = \{A_{1+ (i-2)\pmod n}, A_{(i+1)\pmod n} \mid A_iB \text{ is the extra edge for some vertex }B \}$$

clearly, $|A| \leq 4k$. \\
For any pair of distinct vertices $A$ and $B$, Let $E$ be the point nearest to $A$ such that an extra edge emerges from $E$ i.e. there are no endpoints of extra edges between $A$ and $E$. Now we claim that neighbours of $E$ distinguishes $A$ and $B$. \\
Let the neighbour of $E$ between $A$ and $E$ be $E_1$ and the other one be $E_2$. Let $d_{G'}(A, E) = d$. Clearly, $d_{G'}(A, E_1) = d - 1$ and $d_{G'}(A, E_2) = d + 1$. (\textbf{Should I write the argument here?})\\
Assume that $E_1$ and $E_2$ doesn't distinguish $A$ and $B$. So $d_{G'}(B, E_1) = d - 1$ and $d_{G'}(B, E_2) = d + 1$. Now we try to look at the possible vertices $C$ such that $d_{G'}(B, C) = d - 2$. Knowing that $d_{G'}(B, E_1) = d - 1$, possible candidates for $C$ are $E$ and the other neighbour of $E_1$ as there are no edges emerging between $A$ and $E$. but clearly $E$ is not possible because otherwise $d_{G'}(B, E_2) = d - 1$. This implies that $B$ has to be $d-1$ distance apart from $E_1$ on the ring in the direction of $A$ which means $B = A$ violating that $A$ and $B$ are distinct. \textbf{more rigorous argument and also case when $A = E$, add figure}

\end{proof}
